Spikemax: Spike-based Loss Methods for Classification

Spiking Neural Networks~(SNNs) are a promising research paradigm for low power edge-based computing. Recent works in SNN backpropagation has enabled training of SNNs for practical tasks. However, since spikes are binary events in time, standard loss formulations are not directly compatible with spike output. As a result, current works are limited to using mean-squared loss of spike count. In this paper, we formulate the output probability interpretation from the spike count measure and introduce spike-based negative log-likelihood measure which are more suited for classification tasks especially in terms of the energy efficiency and inference latency. We compare our loss measures with other existing alternatives and evaluate using classification performances on three neuromorphic benchmark datasets: NMNIST, DVS Gesture and N-TIDIGITS18. In addition, we demonstrate state of the art performances on these datasets, achieving faster inference speed and less energy consumption.

==> 04_results/dvsGesture/spikeCount.tex <==
% This file was created by tikzplotlib v0.8.7.
\begin{tikzpicture}

\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.97,0.5)}, anchor=east, draw=white!80.0!black},
legend pos=outer north east,
tick align=outside,
tick pos=both,
x grid style={white!69.01960784313725!black},
xlabel={Spike Count},
xmin=0, xmax=4618599.1273863,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ymin=-0.59, ymax=3.59,
ytick style={color=black},
yticklabels = {, spike-rate, spikemax, spikemax$_g$, spikemax$_s$},
]
\draw[fill=color0,draw opacity=0] (axis cs:0,-0.4) rectangle (axis cs:1358332.7946968,0.4);
\addlegendimage{ybar,ybar legend,fill=color0,draw opacity=0,area legend};
\addlegendentry{layer 0}

\draw[fill=color0,draw opacity=0] (axis cs:0,0.6) rectangle (axis cs:2552460.0689392,1.4);
\draw[fill=color0,draw opacity=0] (axis cs:0,1.6) rectangle (axis cs:1965503.9871212,2.4);
\draw[fill=color0,draw opacity=0] (axis cs:0,2.6) rectangle (axis cs:1218121.897727,3.4);
\draw[fill=color1,draw opacity=0] (axis cs:1358332.7946968,-0.4) rectangle (axis cs:3622817.306818,0.4);
\addlegendimage{ybar,ybar legend,fill=color1,draw opacity=0,area legend};
\addlegendentry{layer 1}

\draw[fill=color1,draw opacity=0] (axis cs:2552460.0689392,0.6) rectangle (axis cs:4237528.4833332,1.4);
\draw[fill=color1,draw opacity=0] (axis cs:1965503.9871212,1.6) rectangle (axis cs:3481596.0757574,2.4);
\draw[fill=color1,draw opacity=0] (axis cs:1218121.897727,2.6) rectangle (axis cs:2779391.0340906,3.4);
\draw[fill=color2,draw opacity=0] (axis cs:3622817.306818,-0.4) rectangle (axis cs:3665715.8363634,0.4);
\addlegendimage{ybar,ybar legend,fill=color2,draw opacity=0,area legend};
\addlegendentry{layer 2}

\draw[fill=color2,draw opacity=0] (axis cs:4237528.4833332,0.6) rectangle (axis cs:4397133.2265152,1.4);
\draw[fill=color2,draw opacity=0] (axis cs:3481596.0757574,1.6) rectangle (axis cs:3604348.9810604,2.4);
\draw[fill=color2,draw opacity=0] (axis cs:2779391.0340906,2.6) rectangle (axis cs:2807428.263636,3.4);
\draw[fill=color3,draw opacity=0] (axis cs:3665715.8363634,-0.4) rectangle (axis cs:3667217.7272724,0.4);
\addlegendimage{ybar,ybar legend,fill=color3,draw opacity=0,area legend};
\addlegendentry{layer 3}

\draw[fill=color3,draw opacity=0] (axis cs:4397133.2265152,0.6) rectangle (axis cs:4398665.835606,1.4);
\draw[fill=color3,draw opacity=0] (axis cs:3604348.9810604,1.6) rectangle (axis cs:3605420.110606,2.4);
\draw[fill=color3,draw opacity=0] (axis cs:2807428.263636,2.6) rectangle (axis cs:2808499.0909086,3.4);
\end{axis}

\end{tikzpicture}


==> 04_results/nmnist/spikeCount.tex <==
% This file was created by tikzplotlib v0.8.7.
\begin{tikzpicture}

\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.97,0.5)}, anchor=east, draw=white!80.0!black},
legend pos=outer north east,
tick align=outside,
tick pos=both,
x grid style={lightgray!92.02614379084967!black},
xlabel={Spike Count},
xmin=0, xmax=650351.194038,
xtick style={color=black},
y grid style={lightgray!92.02614379084967!black},
ymin=-0.59, ymax=3.59,
ytick style={color=black},
yticklabels = {, spike-rate, spikemax, spikemax$_g$, spikemax$_s$},
]
\draw[fill=color0,draw opacity=0] (axis cs:0,-0.4) rectangle (axis cs:212253.52032,0.4);
\addlegendimage{ybar,ybar legend,fill=color0,draw opacity=0,area legend};
\addlegendentry{layer 0}

\draw[fill=color0,draw opacity=0] (axis cs:0,0.6) rectangle (axis cs:86685.08062,1.4);
\draw[fill=color0,draw opacity=0] (axis cs:0,1.6) rectangle (axis cs:98814.88566,2.4);
\draw[fill=color0,draw opacity=0] (axis cs:0,2.6) rectangle (axis cs:77673.88764,3.4);
\draw[fill=color1,draw opacity=0] (axis cs:212253.52032,-0.4) rectangle (axis cs:502579.44674,0.4);
\addlegendimage{ybar,ybar legend,fill=color1,draw opacity=0,area legend};
\addlegendentry{layer 1}

\draw[fill=color1,draw opacity=0] (axis cs:86685.08062,0.6) rectangle (axis cs:291571.08176,1.4);
\draw[fill=color1,draw opacity=0] (axis cs:98814.88566,1.6) rectangle (axis cs:282704.73412,2.4);
\draw[fill=color1,draw opacity=0] (axis cs:77673.88764,2.6) rectangle (axis cs:202829.49932,3.4);
\draw[fill=color2,draw opacity=0] (axis cs:502579.44674,-0.4) rectangle (axis cs:614325.06512,0.4);
\addlegendimage{ybar,ybar legend,fill=color2,draw opacity=0,area legend};
\addlegendentry{layer 2}

\draw[fill=color2,draw opacity=0] (axis cs:291571.08176,0.6) rectangle (axis cs:450624.66358,1.4);
\draw[fill=color2,draw opacity=0] (axis cs:282704.73412,1.6) rectangle (axis cs:409483.8444,2.4);
\draw[fill=color2,draw opacity=0] (axis cs:202829.49932,2.6) rectangle (axis cs:242935.8609,3.4);
\draw[fill=color3,draw opacity=0] (axis cs:614325.06512,-0.4) rectangle (axis cs:619214.0245,0.4);
\addlegendimage{ybar,ybar legend,fill=color3,draw opacity=0,area legend};
\addlegendentry{layer 3}

\draw[fill=color3,draw opacity=0] (axis cs:450624.66358,0.6) rectangle (axis cs:477028.688,1.4);
\draw[fill=color3,draw opacity=0] (axis cs:409483.8444,1.6) rectangle (axis cs:424925.11502,2.4);
\draw[fill=color3,draw opacity=0] (axis cs:242935.8609,2.6) rectangle (axis cs:245403.2347,3.4);
\draw[fill=color4,draw opacity=0] (axis cs:619214.0245,-0.4) rectangle (axis cs:619382.08956,0.4);
\addlegendimage{ybar,ybar legend,fill=color4,draw opacity=0,area legend};
\addlegendentry{layer 4}

\draw[fill=color4,draw opacity=0] (axis cs:477028.688,0.6) rectangle (axis cs:477346.98258,1.4);
\draw[fill=color4,draw opacity=0] (axis cs:424925.11502,1.6) rectangle (axis cs:425119.4518,2.4);
\draw[fill=color4,draw opacity=0] (axis cs:245403.2347,2.6) rectangle (axis cs:245529.4116,3.4);
\end{axis}

\end{tikzpicture}


==> 04_results/ntidigits/spikeCount.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.97,0.5)}, anchor=east, draw=white!80!black},
legend pos=outer north east,
tick align=outside,
tick pos=both,
x grid style={white!69.0196078431373!black},
xlabel={Spike Count},
xmin=0, xmax=105623.07,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=-0.59, ymax=3.59,
ytick style={color=black},
ytick={0,1,2,3},
yticklabels={spike-rate,spikemax,spikemax\(\displaystyle _g\),spikemax\(\displaystyle _s\)}
]
\draw[draw=none,fill=color0] (axis cs:0,-0.4) rectangle (axis cs:17671.4,0.4);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0,area legend};
\addlegendentry{layer 0}

\draw[draw=none,fill=color0] (axis cs:0,0.6) rectangle (axis cs:18538.8,1.4);
\draw[draw=none,fill=color0] (axis cs:0,1.6) rectangle (axis cs:17008.4,2.4);
\draw[draw=none,fill=color0] (axis cs:0,2.6) rectangle (axis cs:6542,3.4);
\draw[draw=none,fill=color1] (axis cs:17671.4,-0.4) rectangle (axis cs:78215.6,0.4);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1,area legend};
\addlegendentry{layer 1}

\draw[draw=none,fill=color1] (axis cs:18538.8,0.6) rectangle (axis cs:95087,1.4);
\draw[draw=none,fill=color1] (axis cs:17008.4,1.6) rectangle (axis cs:88039.2,2.4);
\draw[draw=none,fill=color1] (axis cs:6542,2.6) rectangle (axis cs:9676.6,3.4);
\draw[draw=none,fill=color2] (axis cs:78215.6,-0.4) rectangle (axis cs:79388.4,0.4);
\addlegendimage{ybar,ybar legend,draw=none,fill=color2,area legend};
\addlegendentry{layer 2}

\draw[draw=none,fill=color2] (axis cs:95087,0.6) rectangle (axis cs:100593.4,1.4);
\draw[draw=none,fill=color2] (axis cs:88039.2,1.6) rectangle (axis cs:88492.2,2.4);
\draw[draw=none,fill=color2] (axis cs:9676.6,2.6) rectangle (axis cs:10097.4,3.4);
\end{axis}

\end{tikzpicture}

